Giant planets population around B stars from the first part of the BEAST survey

Exoplanets form from circumstellar protoplanetary discs whose fundamental properties (notably their extent, composition, mass, temperature and lifetime) depend on the host star properties, such as their mass and luminosity. B-stars are among the most massive stars and their protoplanetary discs test extreme conditions for exoplanet formation. This paper investigates the frequency of giant planet companions around young B-stars (median age of 16 Myr) in the Scorpius-Centaurus association, the closest association containing a large population of B-stars. We systematically search for massive exoplanets with the high-contrast direct imaging instrument SPHERE using the data from the BEAST survey, that targets an homogeneous sample of young B-stars from the wide Sco-Cen association. We derive accurate detection limits in case of non-detections. We found evidence in previous papers for two substellar companions around 42 stars. The masses of these companions are straddling the ~13 Jupiter mass deuterium burning limit but their mass ratio with respect to their host star is close to that of Jupiter. We derive a frequency of such massive planetary mass companions around B stars of 11-5+7%, accounting for the survey sensitivity. The discoveries of substellar companions bcen b and mu2sco B happened after only few stars in the survey had been observed, raising the possibility that massive Jovian planets might be common around B-stars. However our statistical analysis show that the occurrence rate of such planets is similar around B-stars and around solar-type stars of similar age, while B-star companions exhibit low mass ratios and larger semi-major axis.

==> notes.tex <==





Panic et al. (2021): two young (2.8, 8 Myr) binary systems with A primaries, secondary with q~0.25-0.7, separations ~250-300 au; both seen by ALMA to possess circumstellar disks. Small disk mass due to mutual photoevaporation

Fontanive+21: census of 938 stars hosting a total of 1316 extra-solar planets and brown dwarf companions, out to 200 pc. A total of 218 planet hosts in multiple-star systems, including 186 binaries and 32 hierarchical triple systems, with 10 newly discovered binary companions and 2 new tertiary components.


after the referee report, it can be good to say in the paper that: "the fact that we have two brown dwarfs, for sure coeval, with very different masses, is a nice way to test the accuracy of evolutionary models" 








